Weak universality in sensory tradeoffs

For many organisms, the number of sensory neurons is largely determined during development, before strong environmental cues are present. This is despite the fact that environments can fluctuate drastically both from generation to generation and within an organism's lifetime. How can organisms get by by hard-coding the number of sensory neurons? We approach this question using rate-distortion theory. A combination of simulation and theory suggests that when environments are large, the rate-distortion function---a proxy for material costs, timing delays, and energy requirements---depends only on coarse-grained environmental statistics that are expected to change on evolutionary, rather than ontogenetic, timescales.

==> cmechabbrev.tex <==
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

% Abbreviations from CMPPSS:

\newcommand{\eM}     {\mbox{$\epsilon$-machine}}
\newcommand{\eMs}    {\mbox{$\epsilon$-machines}}
\newcommand{\EM}     {\mbox{$\epsilon$-Machine}}
\newcommand{\EMs}    {\mbox{$\epsilon$-Machines}}
\newcommand{\eT}     {\mbox{$\epsilon$-transducer}}
\newcommand{\eTs}    {\mbox{$\epsilon$-transducers}}
\newcommand{\ET}     {\mbox{$\epsilon$-Transducer}}

% cryptic
\newcommand{\order}[1]{order\protect\nobreakdash-$#1$}
\newcommand{\Order}[1]{Order\protect\nobreakdash-$#1$}
\newcommand{\cryptic}[1]{$#1$\protect\nobreakdash-cryptic}
\newcommand{\Cryptic}[1]{$#1$\protect\nobreakdash-Cryptic}
\newcommand{\crypticity}[1]{$#1$\protect\nobreakdash-crypticity}
\newcommand{\Crypticity}[1]{$#1$\protect\nobreakdash-Crypticity}

\newcommand{\ETs}    {\mbox{$\epsilon$-Transducers}}

% Processes and sequences

\newcommand{\Process}{\mathcal{P}}

\newcommand{\ProbMach}{\Prob_{\mathrm{M}}}
\newcommand{\Lmax}   { {L_{\mathrm{max}}}}
\newcommand{\MeasAlphabet}  {\mathcal{A}}
% Original symbol
%\newcommand{\MeasSymbol}   { {S} }
%\newcommand{\meassymbol}   { {s} }
% New symbol
\newcommand{\SampleSpace} { \AllPasts }
\newcommand{\MeasSymbol}   { {X} }
\newcommand{\meassymbol}   { {x} }
\newcommand{\MeasSymbols}[2]{ \MeasSymbol_{#1:#2} }
\newcommand{\meassymbols}[2] { \meassymbol_{#1:#2} }
\newcommand{\BiInfinity}    { \smash{\overleftrightarrow {\MeasSymbol}} }
\newcommand{\biinfinity}    { \smash{\overleftrightarrow {\meassymbol}} }
\newcommand{\Past} { \smash{\overleftarrow {\MeasSymbol}} }
%\newcommand{\Past} { \MeasSymbols{}{0} }
\newcommand{\past} { {\smash{\overleftarrow {\meassymbol}}} }
%\newcommand{\past} { \meassymbols{}{0} }
\newcommand{\pastprime} { {\past}^{\prime}}
\newcommand{\Future}   { \smash{\overrightarrow{\MeasSymbol}} }
%\newcommand{\Future} { \MeasSymbols{0}{} }
\newcommand{\future}   { \smash{\overrightarrow{\meassymbol}} }
%\newcommand{\future} { \meassymbols{0}{} }
\newcommand{\futureprime}   { \smash{\future^{\prime}} }
\newcommand{\PastPrime}     { \smash{\Past^{\prime}} }
\newcommand{\FuturePrime}   { \smash{\overrightarrow{\meassymbol}^\prime} }
\newcommand{\PastDblPrime}  { \smash{\overleftarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\FutureDblPrime}{ \smash{\overrightarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\pastL} { \smash{\overleftarrow {\meassymbol}{}^L} }
\newcommand{\PastL} { \smash{\overleftarrow {\MeasSymbol}{}^L} }
\newcommand{\PastLt}      { \smash{\overleftarrow {\MeasSymbol}_t^L} }
\newcommand{\PastLLessOne}{ \smash{\overleftarrow {\MeasSymbol}^{L-1}} }
\newcommand{\futureL}     { \smash{\overrightarrow{\meassymbol}{}^L} }
\newcommand{\FutureL}     { \smash{\overrightarrow{\MeasSymbol}{}^L} }
\newcommand{\FutureLt}    { \smash{\overrightarrow{\MeasSymbol}_t^L} }
\newcommand{\FutureLLessOne}{ \smash{\overrightarrow{\MeasSymbol}^{L-1}} }
\newcommand{\pastLprime}    { \smash{\overleftarrow {\meassymbol}^{L^\prime}} }
\newcommand{\futureLprime}  { \smash{\overrightarrow{\meassymbol}^{L^\prime}} }
\newcommand{\AllPasts}      { \smash{\overleftarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\AllFutures}    { \smash{\overrightarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\FutureSet} { \smash{\overrightarrow{\bf \MeasSymbol}} }
\newcommand{\rep}    { r }
\newcommand{\Rep}    { \mathcal{R} }
\newcommand{\repa}    { \widehat{r} }
\newcommand{\Repa}    { \widehat{\mathcal{R}} }
\newcommand{\repb}    { \widetilde{r} }
\newcommand{\Repb}    { \widetilde{\mathcal{R}} }


\newcommand{\Present} {\MeasSymbol_0}

% Causal states and epsilon-machines
\newcommand{\CausalState}   { \mathcal{S} }
\newcommand{\CausalStatePrime}  { {\CausalState}^{\prime}}
\newcommand{\causalstate}   { \sigma }
\newcommand{\CausalStateSet}    { \bm{\CausalState} }
\newcommand{\AlternateState}    { \mathcal{R} }
\newcommand{\AlternateStatePrime}   { \AlternateState^{\prime} }
\newcommand{\alternatestate}    { \rho }
\newcommand{\alternatestateprime}   { {\rho^{\prime}} }
\newcommand{\AlternateStateSet} { \bm{\AlternateState} }
\newcommand{\PrescientState}    { \widehat{\AlternateState} }
\newcommand{\prescientstate}    { \widehat{\alternatestate} }
\newcommand{\PrescientStateSet} { \bm{\PrescientState}}
\newcommand{\CausalEquivalence} { {\sim}_{\epsilon} }
\newcommand{\CausalEquivalenceNot}  { {\not \sim}_{\epsilon}}

\newcommand{\NonCausalEquivalence}  { {\sim}_{\eta} }
\newcommand{\NextObservable}    { {\smash{\overrightarrow {\MeasSymbol}}^1} }
\newcommand{\LastObservable}    { {\smash{\overleftarrow {\MeasSymbol}}^1} }
%\newcommand{\Prob}     { {\rm P}}
\newcommand{\Prob}      {\Pr} % use standard command
\newcommand{\ProbAnd}   { {,\;} }
\newcommand{\LLimit}    { {L \rightarrow \infty}}
\newcommand{\Cmu}       {C_\mu}
\newcommand{\hmu}       {h_\mu}
\newcommand{\EE}        {{\bf E}}
\newcommand{\TI}        {{\bf T}}
\newcommand{\SI}        {{\bf S}}
\newcommand{\SE}        { H_{\mathrm{sync}} }
\newcommand{\Measurable}{{\bf \mu}}

% Process Crypticity
\newcommand{\PC}        {\chi}

% Causal Irreversibility
\newcommand{\CI}        {\Xi}
\newcommand{\ReverseMap}    {r}
\newcommand{\ForwardMap}    {f}

% Abbreviations from IB:
% None that aren't already in CMPPSS

% Abbreviations from Extensive Estimation:
\newcommand{\EstCausalState}    {\widehat{\CausalState}}
\newcommand{\estcausalstate}    {\widehat{\causalstate}}
\newcommand{\EstCausalStateSet} {\mathbf{\EstCausalState}}
\newcommand{\EstCausalFunc} {\widehat{\epsilon}}
\newcommand{\EstCmu}        {\widehat{\Cmu}}
\newcommand{\PastLOne}  {{\Past}^{L+1}}
\newcommand{\pastLOne}  {{\past}^{L+1}}

% Abbreviations from $\epsilon$-Transducers:
\newcommand{\InAlphabet}    { \mathcal{A}}
\newcommand{\insymbol}      { a}
\newcommand{\OutAlphabet}   { \mathcal{B}}
\newcommand{\outsymbol}     { b}
\newcommand{\InputSimple}   { X}
\newcommand{\inputsimple}   { x}
\newcommand{\BottleneckVar} {\tilde{\InputSimple}}
\newcommand{\bottleneckvar} {\tilde{\inputsimple}}
\newcommand{\InputSpace}    { \mathbf{\InputSimple}}
\newcommand{\InputBi}   { \overleftrightarrow {\InputSimple} }
\newcommand{\inputbi}   { \overleftrightarrow {\inputsimple} }
\newcommand{\InputPast} { \overleftarrow {\InputSimple} }
\newcommand{\inputpast} { \overleftarrow {\inputsimple} }
\newcommand{\InputFuture}   { \overrightarrow {\InputSimple} }
\newcommand{\inputfuture}   { \overrightarrow {\inputsimple} }
\newcommand{\NextInput} { {{\InputFuture}^{1}}}
\newcommand{\NextOutput}    { {\OutputFuture}^{1}}
\newcommand{\OutputSimple}  { Y}
\newcommand{\outputsimple}  { y}
\newcommand{\OutputSpace}   { \mathbf{\OutputSimple}}
\newcommand{\OutputBi}  { \overleftrightarrow{\OutputSimple} }
\newcommand{\outputbi}  { \overleftrightarrow{\outputsimple} }
\newcommand{\OutputPast}    { \overleftarrow{\OutputSimple} }
\newcommand{\outputpast}    { \overleftarrow{\outputsimple} }
\newcommand{\OutputFuture}  { \overrightarrow{\OutputSimple} }
\newcommand{\outputfuture}  { \overrightarrow{\outputsimple} }
\newcommand{\OutputL}   { {\OutputFuture}^L}
\newcommand{\outputL}   { {\outputfuture}^L}
\newcommand{\InputLLessOne} { {\InputFuture}^{L-1}}
\newcommand{\inputLlessone} { {\inputufutre}^{L-1}}
\newcommand{\OutputPastLLessOne}    {{\OutputPast}^{L-1}_{-1}}
\newcommand{\outputpastLlessone}    {{\outputpast}^{L-1}}
\newcommand{\OutputPastLessOne} {{\OutputPast}_{-1}}
\newcommand{\outputpastlessone} {{\outputpast}_{-1}}
\newcommand{\OutputPastL}   {{\OutputPast}^{L}}
\newcommand{\OutputLPlusOne}    { {\OutputFuture}^{L+1}}
\newcommand{\outputLplusone}    { {\outputfutre}^{L+1}}
\newcommand{\InputPastL}    {{\InputPast}^{L}}
\newcommand{\inputpastL}    {{\inputpast}^{L}}
\newcommand{\JointPast} {{(\InputPast,\OutputPast)}}
\newcommand{\jointpast} {{(\inputpast,\outputpast)}}
\newcommand{\jointpastone}  {{(\inputpast_1,\outputpast_1)}}
\newcommand{\jointpasttwo}  {{(\inputpast_2,\outputpast_2)}}
\newcommand{\jointpastprime} {{({\inputpast}^{\prime},{\outputpast}^{\prime})}}
\newcommand{\NextJoint} {{(\NextInput,\NextOutput)}}
\newcommand{\nextjoint} {{(\insymbol,\outsymbol)}}
\newcommand{\AllInputPasts} { { \overleftarrow {\rm \InputSpace}}}
\newcommand{\AllOutputPasts}    { {\overleftarrow {\rm \OutputSpace}}}
\newcommand{\DetCausalState}    { {{\cal S}_D }}
\newcommand{\detcausalstate}    { {{\sigma}_D} }
\newcommand{\DetCausalStateSet} { \mathbf{{\CausalState}_D}}
\newcommand{\DetCausalEquivalence}  { {\sim}_{{\epsilon}_{D}}}
\newcommand{\PrescientEquivalence}  { {\sim}_{\widehat{\eta}}}
\newcommand{\FeedbackCausalState}   { \mathcal{F}}
\newcommand{\feedbackcausalstate}   { \phi}
\newcommand{\FeedbackCausalStateSet}    { \mathbf{\FeedbackCausalState}}
\newcommand{\JointCausalState}      { \mathcal{J}}
\newcommand{\JointCausalStateSet}   { \mathbf{\JointCausalState}}
\newcommand{\UtilityFunctional} { {\mathcal{L}}}
\newcommand{\NatureState}   { {\Omega}}
\newcommand{\naturestate}   { {\omega}}
\newcommand{\NatureStateSpace}  { {\mathbf{\NatureState}}}
\newcommand{\AnAction}  { {A}}
\newcommand{\anaction}  { {a}}
\newcommand{\ActionSpace}   { {\mathbf{\AnAction}}}

% Abbreviations from RURO:
\newcommand{\InfoGain}[2] { \mathcal{D} \left( {#1} || {#2} \right) }

% Abbreviations from Upper Bound:
\newcommand{\lcm}   {{\rm lcm}}
% Double-check that this isn't in the math set already!

% Abbreviations from Emergence in Space
\newcommand{\ProcessAlphabet}   {\MeasAlphabet}
\newcommand{\ProbEst}           { {\widehat{\Prob}_N}}
\newcommand{\STRegion}          { {\mathrm K}}
\newcommand{\STRegionVariable}      { K}
\newcommand{\stregionvariable}      { k}
\newcommand{\GlobalPast}        { \overleftarrow{G}}
\newcommand{\globalpast}        { \overleftarrow{g}}
\newcommand{\GlobalFuture}      { \overrightarrow{G}}
\newcommand{\globalfuture}      { \overrightarrow{g}}
\newcommand{\GlobalState}       { \mathcal{G}}
\newcommand{\globalstate}       { \gamma}
\newcommand{\GlobalStateSet}        { {\mathbf \GlobalState}}
\newcommand{\LocalPast}         { \overleftarrow{L}}
\newcommand{\localpast}         { \overleftarrow{l}}
\newcommand{\AllLocalPasts}     { \mathbf{\LocalPast}}
\newcommand{\LocalPastRegion}       { \overleftarrow{\mathrm L}}
\newcommand{\LocalFuture}       { \overrightarrow{L}}
\newcommand{\localfuture}       { \overrightarrow{l}}
\newcommand{\LocalFutureRegion}     { \overrightarrow{\mathrm L}}
\newcommand{\LocalState}        { \mathcal{L}}
\newcommand{\localstate}        { \lambda}
\newcommand{\LocalStateSet}     { {\mathbf \LocalState}}
\newcommand{\PatchPast}         { \overleftarrow{P}}
\newcommand{\patchpast}         { \overleftarrow{p}}
\newcommand{\PatchPastRegion}       { \overleftarrow{\mathrm P}}
\newcommand{\PatchFuture}       { \overrightarrow{P}}
\newcommand{\patchfuture}       { \overrightarrow{p}}
\newcommand{\PatchFutureRegion}     { \overrightarrow{\mathrm P}}
\newcommand{\PatchState}        { \mathcal{P}}
\newcommand{\patchstate}        { \pi}
\newcommand{\PatchStateSet}     { {\mathbf \PatchState}}
\newcommand{\LocalStatesInPatch}    {\vec{\LocalState}}
\newcommand{\localstatesinpatch}    {\vec{\localstate}}
\newcommand{\PointInstantX}     { {\mathbf x}}
% Galles's original LaTeX for the cond. indep. symbol follows:
\newcommand{\compos}{\mbox{$~\underline{~\parallel~}~$}}
\newcommand{\ncompos}{\not\hspace{-.15in}\compos}
\newcommand{\indep}         { \rotatebox{90}{$\models$}}
\newcommand{\nindep}    {\not\hspace{-.05in}\indep}
\newcommand{\LocalEE}   {{\EE}^{loc}}
\newcommand{\EEDensity} {\overline{\LocalEE}}
\newcommand{\LocalCmu}  {{\Cmu}^{loc}}
\newcommand{\CmuDensity}    {\overline{\LocalCmu}}

%%%%%%%%%%% added by sasa
\newcommand{\FinPast}[1]    { \overleftarrow {\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finpast}[1]    { \overleftarrow {\meassymbol}  \stackrel{{#1}}{}}
\newcommand{\FinFuture}[1]      { \overrightarrow{\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finfuture}[1]      { \overrightarrow{\meassymbol} \stackrel{{#1}}{}}

\newcommand{\Partition} { \AlternateState }
\newcommand{\partitionstate}    { \alternatestate }
\newcommand{\PartitionSet}  { \AlternateStateSet }
\newcommand{\Fdet}   { F_{\rm det} }

\newcommand{\Dkl}[2] { D_{\rm KL} \left( {#1} || {#2} \right) }

\newcommand{\Period}    {p}

% To take into account time direction
\newcommand{\forward}{+}
\newcommand{\reverse}{-}
%\newcommand{\forwardreverse}{\:\!\diamond} % \pm
\newcommand{\forwardreverse}{\pm} % \pm
\newcommand{\FutureProcess} { {\Process}^{\forward} }
\newcommand{\PastProcess}   { {\Process}^{\reverse} }
\newcommand{\FutureCausalState} { {\CausalState}^{\forward} }
\newcommand{\futurecausalstate} { \sigma^{\forward} }
\newcommand{\altfuturecausalstate}  { \sigma^{\forward\prime} }
\newcommand{\PastCausalState}   { {\CausalState}^{\reverse} }
\newcommand{\pastcausalstate}   { \sigma^{\reverse} }
\newcommand{\BiCausalState}     { {\CausalState}^{\forwardreverse} }
\newcommand{\bicausalstate}     { {\sigma}^{\forwardreverse} }
\newcommand{\FutureCausalStateSet}  { {\CausalStateSet}^{\forward} }
\newcommand{\PastCausalStateSet}    { {\CausalStateSet}^{\reverse} }
\newcommand{\BiCausalStateSet}  { {\CausalStateSet}^{\forwardreverse} }
\newcommand{\eMachine}  { M }
\newcommand{\FutureEM}  { {\eMachine}^{\forward} }
\newcommand{\PastEM}    { {\eMachine}^{\reverse} }
\newcommand{\BiEM}      { {\eMachine}^{\forwardreverse} }
\newcommand{\BiEquiv}   { {\sim}^{\forwardreverse} }
\newcommand{\Futurehmu} { h_\mu^{\forward} }
\newcommand{\Pasthmu}   { h_\mu^{\reverse} }
\newcommand{\FutureCmu} { C_\mu^{\forward} }
\newcommand{\PastCmu}   { C_\mu^{\reverse} }
\newcommand{\BiCmu}     { C_\mu^{\forwardreverse} }
\newcommand{\FutureEps} { \epsilon^{\forward} }
\newcommand{\PastEps}   { \epsilon^{\reverse} }
\newcommand{\BiEps} { \epsilon^{\forwardreverse} }
\newcommand{\FutureSim} { \sim^{\forward} }
\newcommand{\PastSim}   { \sim^{\reverse} }
\newcommand{\FuturePC}  {\PC^{\forward}}
\newcommand{\PastPC}        {\PC^{\reverse}}
\newcommand{\BiPC}      {\PC^{\forwardreverse}}

% Used arrows for awhile, more or less confusing?
%\newcommand{\FutureCausalState}    { \overrightarrow{\CausalState} }
%\newcommand{\PastCausalState}  { \overleftarrow{\CausalState} }
%\newcommand{\eMachine} { M }
%\newcommand{\FutureEM} { \overrightarrow{\eMachine} }
%\newcommand{\PastEM}   { \overleftarrow{\eMachine} }
%\newcommand{\FutureCmu}    { \overrightarrow{\Cmu} }
%\newcommand{\PastCmu}  { \overleftarrow{\Cmu} }

%% time-reversing and mixed state presentation operators
\newcommand{\TR}{\mathcal{T}}
\newcommand{\MSP}{\mathcal{U}}
\newcommand{\one}{\mathbf{1}}

%% added for RURO2
%% Note that it will always be typesett in math mode.
%% Example usage:
%%    The 3-block entropy is \BE[t]{3}.
%%    The 3-block-state entropy from $t=0$ is $\BSE{3}$.
%%
%% The optional argument specifies the start time, defaulting to t=0.
%% The mandatory argument specifies the length of the block (not the stop time).
\newcommand{\lastindex}[2]{
  \edef\tempa{0}
  \edef\tempb{#2}
  \ifx\tempa\tempb
    % if the length is 0, then the final time equals the start time
    \edef\tempc{#1}
  \else
    % if the start time is different from zero, then we show the sum
    \edef\tempa{0}
    \edef\tempb{#1}
    \ifx\tempa\tempb
      \edef\tempc{#2}
    \else
      \edef\tempc{#1+#2}
    \fi
  \fi
  \tempc
}
\newcommand{\BE}[2][0]{
  \ensuremath{H[\MeasSymbols{#1}{#2}]}
}
\newcommand{\BSE}[2][0]{
  \ensuremath{H[\MeasSymbols{#1}{#2},\CausalState_{\lastindex{#1}{#2}}]}
}
\newcommand{\SBE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbols{#1}{#2}]}
}
\newcommand{\SBSE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbols{#1}{#2},
                \CausalState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbols{#1}{#2}]}
}
\newcommand{\AltBSE}[2][0]{
  \ensuremath{H[\MeasSymbols{#1}{#2},\AlternateState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBSE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbols{#1}{#2},
                \AlternateState_{\lastindex{#1}{#2}}]}
}
\newcommand{\SGBE}[2][0]{
  \ensuremath{H[\CausalState_{#2} | \MeasSymbols{#1}{#2}]}
}

\newcommand{\GI}{\varphi}
\newcommand{\OI}{\zeta}
% cryptic, gauge, oracular, Markov, and synchronization
\newcommand{\COrder}{k_{\PC}}
\newcommand{\GOrder}{k_{\GI}}
\newcommand{\OOrder}{k_{\OI}}
\newcommand{\MOrder}{R}
\newcommand{\SOrder}{k_{\SI}}
\newcommand{\Lsync} {\mathcal{L}_{\mathrm{sync}}}

%% stuff for the anatomy paper

\newcommand{\rhomu}{\rho_\mu}
\newcommand{\rmu}{r_\mu}
\newcommand{\bmu}{b_\mu}
\newcommand{\qmu}{q_\mu}
\newcommand{\wmu}{w_\mu}
\newcommand{\imu}{i_\mu}
\newcommand{\sigmamu}{\sigma_\mu}
\newcommand{\EER}{\EE_R}
\newcommand{\EEB}{\EE_B}
\newcommand{\EEQ}{\EE_Q}
\newcommand{\EEW}{\EE_W}
\newcommand{\I}{\mathbf{I}}

%% Added to standardize the order of causal states
%% Example usage:
%%    $\BiCmu = H[\CSjoint] = H[\CSjoint[,]]$
%%    $\EE = I[\CSjoint[:]] = I[\CSjoint[;]]$
\newcommand{\CSjoint}[1][,]{
   \edef\tempa{:}
   \edef\tempb{#1}
   \ifx\tempa\tempb
      % arg1 was a colon, insert a small negative space
      \ensuremath{\FutureCausalState\!#1\PastCausalState}
   \else
      % arg1 was not a colon, usually a comma or semicolon
      \ensuremath{\FutureCausalState#1\PastCausalState}
   \fi
}

%% (cje)
%% Provide a command \ifpm which is true when \pm
%% is meant to be understood as "+ or -", opposed
%% to "bidirectional". This differs from the usage
%% in TBA.  Essentially, if \forwardreverse is defined
%% as something different, perhaps a \diamond, then
%% we are free to interpret \pm as "+ or -".
\newif\ifpm
\edef\tempa{\forwardreverse}
\edef\tempb{\pm}
\ifx\tempa\tempb
   \pmfalse
\else
   \pmtrue
\fi




